Applications of Generative Adversarial Networks in Anomaly Detection: A Systematic Literature Review

Anomaly detection has become an indispensable tool for modern society, applied in a wide range of applications, from detecting fraudulent transactions to malignant brain tumours. Over time, many anomaly detection techniques have been introduced. However, in general, they all suffer from the same problem: a lack of data that represents anomalous behaviour. As anomalous behaviour is usually costly (or dangerous) for a system, it is difficult to gather enough data that represents such behaviour. This, in turn, makes it difficult to develop and evaluate anomaly detection techniques. Recently, generative adversarial networks (GANs) have attracted a great deal of attention in anomaly detection research, due to their unique ability to generate new data. In this paper, we present a systematic literature review of the applications of GANs in anomaly detection, covering 128 papers on the subject. The goal of this review paper is to analyze and summarize: (1) which anomaly detection techniques can benefit from certain types of GANs, and how, (2) in which application domains GAN-assisted anomaly detection techniques have been applied, and (3) which datasets and performance metrics have been used to evaluate these techniques. Our study helps researchers and practitioners to find the most suitable GAN-assisted anomaly detection technique for their application. In addition, we present a research roadmap for future studies in this area.

==> Sections/Abstract.tex <==
Anomaly detection has become an indispensable tool for modern society, applied in a wide range of applications, from detecting fraudulent transactions to malignant brain tumours. 
Over time, many anomaly detection techniques have been introduced. However, in general, they all suffer from the same problem: a lack of data that represents anomalous behaviour. As anomalous behaviour is usually costly (or dangerous) for a system, it is difficult to gather enough data that represents such behaviour. This, in turn, makes it difficult to develop and evaluate anomaly detection techniques.
Recently, generative adversarial networks (GANs) have attracted a great deal of attention in anomaly detection research, due to their unique ability to generate new data. In this paper, we
present a systematic literature review of the applications of GANs in anomaly detection, covering 128 papers on the subject.
The goal of this review paper is to analyze and summarize: (1)~which anomaly detection techniques can benefit from certain types of GANs, and how, (2)~in which application domains GAN-assisted anomaly detection techniques have been applied, and (3)~which datasets and performance metrics have been used to evaluate these techniques. Our study helps researchers and practitioners to find the most suitable GAN-assisted anomaly detection technique for their application. In addition, we present a research roadmap for future studies in this area.

==> Sections/PrimaryStudies.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'

  \centering
  \tiny

    \begin{longtable}{|c|l|c|c|}
    \caption{Summary of publications.}\\
    \toprule
    \textbf{Study ID} & \textbf{Title} & \textbf{Database} & \textbf{Pub. Type} \\
    \midrule
    ADG01~\cite{ADG01} & IGAN-IDS: An imbalanced generative adversarial network towards intrusion detection system in ad-hoc networks & Science Direct & Journal \\
    \midrule
    ADG02~\cite{ADG02} & Oversampling method using outlier detectable generative adversarial network & Science Direct & Journal \\
    \midrule
    ADG03~\cite{ADG03} & Exploiting the generative adversarial framework for one-class multi-dimensional fault detection & Science Direct & Journal \\
    \midrule
    ADG04~\cite{ADG04} & f-AnoGAN: Fast unsupervised anomaly detection with generative adversarial networks & Science Direct & Journal \\
    \midrule
    ADG05~\cite{ADG05} & Android-GAN: Defending against android pattern attacks using multi-modal generative network as anomaly detector & Science Direct & Journal \\
    \midrule
    ADG06~\cite{ADG06} & Unsupervised automatic seizure detection for focal-onset seizures recorded with behind-the-ear EEG using an anomaly-detecting generative adversarial network & Science Direct & Journal \\
    \midrule
    ADG07~\cite{ADG07} & Energy theft detection in an edge data center using threshold-based abnormality detector & Science Direct & Journal \\
    \midrule
    ADG08~\cite{ADG08} & A System for Spatiotemporal Anomaly Localization in Surveillance Videos & ACM   & Conference \\
    \midrule
    ADG09~\cite{ADG09} & PredGAN: A Deep Multi-Scale Video Prediction Framework for Detecting Anomalies in Videos & ACM   & Conference \\
    \midrule
    ADG10~\cite{ADG10} & Deep Learning-Based Model to Fight Against Ad Click Fraud & ACM   & Conference \\
    \midrule
    ADG11~\cite{ADG11} & Spatial Temporal Balanced Generative Adversarial AutoEncoder for Anomaly Detection & ACM   & Conference \\
    \midrule
    ADG12~\cite{ADG12} & Driving Anomaly Detection with Conditional Generative Adversarial Network Using Physiological and CAN-Bus Data & ACM   & Conference \\
    \midrule
    ADG13~\cite{ADG13} & Anomaly Detection in Traffic Surveillance Videos with GAN-Based Future Frame Prediction & ACM   & Conference \\
    \midrule
    ADG14~\cite{ADG14} & One-Class Classification with Deep Adversarial Learning & ACM   & Conference \\
    \midrule
    ADG15~\cite{ADG15} & Bypassing Detection of URL-Based Phishing Attacks Using Generative Adversarial Deep Neural Networks & ACM   & Workshop \\
    \midrule
    ADG16~\cite{ADG16} & Coupled IGMM-GANs with Applications to Anomaly Detection in Human Mobility Data & ACM   & Journal \\
    \midrule
    ADG17~\cite{ADG17} & Data Augmentation Using Generative Adversarial Networks for Electrical Insulator Anomaly Detection & ACM   & Conference \\
    \midrule
    ADG18~\cite{ADG18} & Sparse-Gan: Sparsity-Constrained Generative Adversarial Network for Anomaly Detection in Retinal OCT Image & IEEE  & Symposium \\
    \midrule
    ADG19~\cite{ADG19} & Anomaly Generation Using Generative Adversarial Networks in Host-Based Intrusion Detection & IEEE  & Conference \\
    \midrule
    ADG20~\cite{ADG20} & Anomaly Monitoring Framework in Lane Detection With a Generative Adversarial Network & IEEE  & Journal \\
    \midrule
    ADG21~\cite{ADG21} & Semisupervised Spectral Learning With Generative Adversarial Network for Hyperspectral Anomaly Detection & IEEE  & Journal \\
    \midrule
    ADG22~\cite{ADG22} & Generative Adversarial Network Based Anomaly Detection on the Benchmark Tennessee Eastman Process & IEEE  & Conference \\
    \midrule
    ADG23~\cite{ADG23} & Memory-Augmented Anomaly Generative Adversarial Network for Retinal OCT Images Screening & IEEE  & Symposium \\
    \midrule
    ADG24~\cite{ADG24} & Anomaly Detection in Time Series using Generative Adversarial Networks & IEEE  & Conference \\
    \midrule
    ADG25~\cite{ADG25} & Finding Anomalies with Generative Adversarial Networks for a Patrolbot & IEEE  & Conference \\
    \midrule
    ADG26~\cite{ADG26} & Anomaly Detection of Railway Catenary Based on Deep Convolutional Generative Adversarial Networks & IEEE  & Conference \\
    \midrule
    ADG27~\cite{ADG27} & Generative Adversarial Networks For Launching and Thwarting Adversarial Attacks on Network Intrusion Detection Systems & IEEE  & Conference \\
    \midrule
    ADG28~\cite{ADG28}& Interpreting Abnormality of a Complex Static Scene using Generative Adversarial Network & IEEE  & Conference \\
    \midrule
    ADG29~\cite{ADG29} & A Generative Adversarial Network Based Framework for Unsupervised Visual Surface Inspection & IEEE  & Conference \\
    \midrule
    ADG30~\cite{ADG30} & Generative Adversarial Networks (GAN) based Anomaly Detection in Industrial Software Systems & IEEE  & Conference \\
    \midrule
    ADG31~\cite{ADG31} & A Generic Anomaly Detection of Catenary Support Components Based on Generative Adversarial Networks & IEEE  & Journal \\
    \midrule
    ADG32~\cite{ADG32} & Discriminative Reconstruction Constrained Generative Adversarial Network for Hyperspectral Anomaly Detection & IEEE  & Journal \\
    \midrule
    ADG33~\cite{ADG33} & What goes around comes around: Cycle-Consistency-based Short-Term Motion Prediction for Anomaly Detection using Generative Adversarial Networks & IEEE  & Conference \\
    \midrule
    ADG34~\cite{ADG34} & Anomaly Detection via Minimum Likelihood Generative Adversarial Networks & IEEE  & Conference \\
    \midrule
    ADG35~\cite{ADG35} & Anomaly Event Detection Using Generative Adversarial Network for Surveillance Videos & IEEE  & Conference \\
    \midrule
    ADG36~\cite{ADG36} & Industrial Anomaly Detection and One-class Classification using Generative Adversarial Networks & IEEE  & Conference \\
    \midrule
    ADG37~\cite{ADG37} & Dual Discriminator Generative Adversarial Network for Video Anomaly Detection & IEEE  & Journal \\
    \midrule
    ADG38~\cite{ADG38} & Unsupervised Multi-Discriminator Generative Adversarial Network for Lung Nodule Malignancy Classification & IEEE  & Journal \\
    \midrule
    ADG39~\cite{ADG39} & 3D Convolutional Generative Adversarial Networks for Detecting Temporal Irregularities in Videos & IEEE  & Conference \\
    \midrule
    ADG40~\cite{ADG40} & Visual Detection of Generic Defects in Industrial Components using Generative Adversarial Networks & IEEE  & Conference \\
    \midrule
    ADG41~\cite{ADG41} & Stock Price Manipulation Detection using Generative Adversarial Networks & IEEE  & Symposium \\
    \midrule
    ADG42~\cite{ADG42} & Generative Adversarial Networks for Distributed Intrusion Detection in the Internet of Things & IEEE  & Conference \\
    \midrule
    ADG43~\cite{ADG43} & Coupled IGMM-GANs for improved generative adversarial anomaly detection & IEEE  & Conference \\
    \midrule
    ADG44~\cite{ADG44} & Survey on Applying GAN for Anomaly Detection & IEEE  & Conference \\
    \midrule
    ADG45~\cite{ADG45} & GAN-Based Anomaly Detection and Localization of Multivariate Time Series Data for Power Plant & IEEE  & Conference \\
    \midrule
    ADG46~\cite{ADG46} & A GAN-Based Anomaly Detection Method for Isoelectric Line in High-Speed Railway & IEEE  & Conference \\
    \midrule
    ADG47~\cite{ADG47} & Mahalanobis Distance Based Adversarial Network for Anomaly Detection & IEEE  & Conference \\
    \midrule
    ADG48~\cite{ADG48} & Fence GAN: Towards Better Anomaly Detection & IEEE  & Conference \\
    \midrule
    ADG49~\cite{ADG49} & A Novel LSTM-GAN Algorithm for Time Series Anomaly Detection & IEEE  & Conference \\
    \midrule
    ADG50~\cite{ADG50} & A GAN-Based Anomaly Detection Approach for Imbalanced Industrial Time Series & IEEE  & Journal \\
    \midrule
    ADG51~\cite{ADG51} & Enhanced Adversarial Learning Based Video Anomaly Detection with Object Confidence and Position & IEEE  & Conference \\
    \midrule
    ADG52~\cite{ADG52} & ADGAN: A Scalable GAN-based Architecture for Image Anomaly Detection & IEEE  & Conference \\
    \midrule
    ADG53~\cite{ADG53} & Generative Adversarial Active Learning for Unsupervised Outlier Detection & IEEE  & Journal \\
    \midrule
    ADG54~\cite{ADG54} & Learning-Based Real-Time Process-Aware Anomaly Monitoring for Assured Autonomy & IEEE  & Journal \\
    \midrule
    ADG55~\cite{ADG55} & Lifelong Disk Failure Prediction via GAN-Based Anomaly Detection & IEEE  & Conference \\
    \midrule
    ADG56~\cite{ADG56} & A Semi-supervised Approach for Steam Turbine Health Prognostics Based on GAN and PF & IEEE  & Conference \\
    \midrule
    ADG57~\cite{ADG57} & Abnormal Chest X-Ray Identification With Generative Adversarial One-Class Classifier & IEEE  & Symposium \\
    \midrule
    ADG58~\cite{ADG58} & Time Series Anomaly Detection Based on GAN & IEEE  & Conference \\
    \midrule
    ADG59~\cite{ADG59} & Anomaly Dataset Augmentation Using the Sequence Generative Models & IEEE  & Conference \\
    \midrule
    ADG60~\cite{ADG60} & Adversarially Learned Abnormal Trajectory Classifier & IEEE  & Conference \\
    \midrule
    ADG61~\cite{ADG61} & Adversarially Learned Anomaly Detection & IEEE  & Conference \\
    \midrule
    ADG62~\cite{ADG62} & A Novel and Efficient CVAE-GAN-Based Approach With Informative Manifold for Semi-Supervised Anomaly Detection & IEEE  & Journal \\
    \midrule
    ADG63~\cite{ADG63} & Training Adversarial Discriminators for Cross-Channel Abnormal Event Detection in Crowds & IEEE  & Conference \\
    \midrule
    ADG64~\cite{ADG64} & Unsupervised Anomaly Detection and Localization Based on Deep Spatiotemporal Translation Network & IEEE  & Journal \\
    \midrule
    ADG65~\cite{ADG65} & MVTec AD — A Comprehensive Real-World Dataset for Unsupervised Anomaly Detection & IEEE  & Conference \\
    \midrule
    ADG66~\cite{ADG66} & Deep Embedding GAN-based Model for Anomaly Detection on High-dimensional Sparse Data & IEEE  & Conference \\
    \midrule
    ADG67~\cite{ADG67} & Robust and Computationally-Efficient Anomaly Detection Using Powers-Of-Two Networks & IEEE  & Conference \\
    \midrule
    ADG68~\cite{ADG68} & GAN Augmented Text Anomaly Detection with Sequences of Deep Statistics & IEEE  & Conference \\
    \midrule
    ADG69~\cite{ADG69} & Abnormal Colon Polyp Image Synthesis Using Conditional Adversarial Networks for Improved Detection Performance & IEEE  & Journal \\
    \midrule
    ADG70~\cite{ADG70} & Defect Image Sample Generation With GAN for Improving Defect Recognition & IEEE  & Journal \\
    \midrule
    ADG71~\cite{ADG71} & Steel Surface Defect Detection Using GAN and One-Class Classifier & IEEE  & Conference \\
    \midrule
    ADG72~\cite{ADG72} & Generative And Encoded Anomaly Detectors & IEEE  & Workshop \\
    \midrule
    ADG73~\cite{ADG73} & Discriminative Autoencoding Framework for Simple and Efficient Anomaly Detection & IEEE  & Journal \\
    \midrule
    ADG74~\cite{ADG74} & Deep Learning Based Fusion of RGB and Infrared Images for the Detection of Abnormal Condition of Fused Magnesium Furnace & IEEE  & Conference \\
    \midrule
    ADG75~\cite{ADG75} & a Multi-Perspective Approach to Anomaly Detection for Self-Aware Embodied Agents & IEEE  & Conference \\
    \midrule
    ADG76~\cite{ADG76} & High Performance WGAN-GP based Multiple-category Network Anomaly Classification System & IEEE  & Conference \\
    \midrule
    ADG77~\cite{ADG77} & Self-Secured Control with Anomaly Detection and Recovery in Automotive Cyber-Physical Systems & IEEE  & Conference \\
    \midrule
    ADG78~\cite{ADG78} & Abnormal event detection in videos using generative adversarial nets & IEEE  & Conference \\
    \midrule
    ADG79~\cite{ADG79} & Learning Normal Patterns via Adversarial Attention-based Autoencoder for Abnormal Event Detection in Videos & IEEE  & Journal \\
    \midrule
    ADG80~\cite{ADG80} & AI-Based Abnormality Detection at the PHY-Layer of Cognitive Radio by Learning Generative Models & IEEE  & Journal \\
    \midrule
    ADG81~\cite{ADG81} & Image-based Process Monitoring via Adversarial Autoencoder with Applications to Rolling Defect Detection & IEEE  & Journal \\
    \midrule
    ADG82~\cite{ADG82} & Bone Metastatic Tumor Detection based on AnoGAN Using CT Images & IEEE  & Conference \\
    \midrule
    ADG83~\cite{ADG83} & Credit Card Transactions Data Adversarial Augmentation in the Frequency Domain & IEEE  & Conference \\
    \midrule
    ADG84~\cite{ADG84} & Data Expansion for Foreign Object Detection in Power Grid & IEEE  & Conference \\
    \midrule
    ADG85~\cite{ADG85} & Adversarially Learned One-Class Classifier for Novelty Detection & IEEE  & Conference \\
    \midrule
    ADG86~\cite{ADG86} & An Adversarial Learning Approach to Medical Image Synthesis for Lesion Detection & IEEE  & Journal \\
    \midrule
    ADG87~\cite{ADG87} & Photoshopping Colonoscopy Video Frames & IEEE  & Symposium \\
    \midrule
    ADG88~\cite{ADG88} & End-to-End Adversarial Learning for Intrusion Detection in Computer Networks & IEEE  & Conference \\
    \midrule
    ADG89~\cite{ADG89} & Assessment of Data Augmentation Strategies Toward Performance Improvement of Abnormality Classification in Chest Radiographs & IEEE  & Conference \\
    \midrule
    ADG90~\cite{ADG90} & Deep detector classifier (DeepDC) for moving objects segmentation and classification in video surveillance & IEEE  & Journal \\
    \midrule
    ADG91~\cite{ADG91} & Multi-sensor Fusion for Magnetic Flux Leakage Defect Characterization Under Information Incompletion & IEEE  & Journal \\
    \midrule
    ADG92~\cite{ADG92} & A Simple Recurrent Unit Model Based Intrusion Detection System With DCGAN & IEEE  & Journal \\
    \midrule
    ADG93~\cite{ADG93} & Relativistic Discriminator: A One-Class Classifier for Generalized Iris Presentation Attack Detection & IEEE  & Conference \\
    \midrule
    ADG94~\cite{ADG94} & Unsupervised Protocol-based Intrusion Detection for Real-world Networks & IEEE  & Conference \\
    \midrule
    ADG95~\cite{ADG95} & An automobile environment detection system based on deep neural network and its implementation using iot-enabled in-vehicle air quality sensors & Scopus & Journal \\
    \midrule
    ADG96~\cite{ADG96} & Unsupervised Anomaly Detection of Healthcare Providers Using Generative Adversarial Networks & Scopus & Conference \\
    \midrule
    ADG97~\cite{ADG97} & video anomaly detection in post-procedural use of laparoscopic videos & Scopus & Workshop \\
    \midrule
    ADG98~\cite{ADG98} & GAN-based Abnormal Detection by Recognizing Ungeneratable Patterns & Scopus & Conference \\
    \midrule
    ADG99~\cite{ADG99} & Semi-supervised Deep Learning for Network Anomaly Detection & Scopus & Conference \\
    \midrule
    ADG100~\cite{ADG100} & MimicGAN: Robust Projection onto Image Manifolds with Corruption Mimicking & Scopus & Journal \\
    \midrule
    ADG101~\cite{ADG101} & Perceptual Image Anomaly Detection & Scopus & Conference \\
    \midrule
    ADG102~\cite{ADG102} & Abnormal Event Detection and Localization in Visual Surveillance & Scopus & Conference \\
    \midrule
    ADG103~\cite{ADG103} & A new GAN-based anomaly detection (GBAD) approach for multi-threat object classification on large-scale x-ray security images & Scopus & Journal \\
    \midrule
    ADG104~\cite{ADG104} & Early Detection of Tomato Spotted Wilt Virus by Hyperspectral Imaging and Outlier Removal Auxiliary Classifier Generative Adversarial Nets (OR-AC-GAN) & Scopus & Journal \\
    \midrule
    ADG105~\cite{ADG105} & Unsupervised anomaly detection system for railway turnout based on GAN & Scopus & Conference \\
    \midrule
    ADG106~\cite{ADG106} & AE-CGAN model based high performance network intrusion detection system & Scopus & Journal \\
    \midrule
    ADG107~\cite{ADG107} & Breast cancer detection using synthetic mammograms from generative adversarial networks in convolutional neural networks & Scopus & Journal \\
    \midrule
    ADG108~\cite{ADG108} & MAD-GAN: Multivariate Anomaly Detection for Time Series Data with Generative Adversarial Networks & Scopus & Conference \\
    \midrule
    ADG109~\cite{ADG109} & LogGAN: A Sequence-Based Generative Adversarial Network for Anomaly Detection Based on System Logs & Scopus & Conference \\
    \midrule
    ADG110~\cite{ADG110} & Image anomaly detection with generative adversarial networks & Scopus & Conference \\
    \midrule
    ADG111~\cite{ADG111} & Few-shot learning with generative adversarial networks based on WOA13 data & Scopus & Journal \\
    \midrule
    ADG112~\cite{ADG112} & Using generative adversarial networks and transfer learning for breast cancer detection by convolutional neural networks & Scopus & Conference \\
    \midrule
    ADG113~\cite{ADG113} & GANomaly: Semi-supervised Anomaly Detection via Adversarial Training & Scopus & Conference \\
    \midrule
    ADG114~\cite{ADG114} & Deep adversarial one-class learning for normal and abnormal chest radiograph classification & Scopus & Conference \\
    \midrule
    ADG115~\cite{ADG115} & Semi-supervised VAE-GAN for Out-of-Sample Detection Applied to MRI Quality Control & Scopus & Conference \\
    \midrule
    ADG116~\cite{ADG116} & Deep learning for automated defect detection in high-reliability electronic parts & Scopus & Conference \\
    \midrule
    ADG117~\cite{ADG117} & Detecting Anomalies in Communication Packet Streams Based on Generative Adversarial Networks & Scopus & Conference \\
    \midrule
    ADG118~\cite{ADG118} & AVID: Adversarial Visual Irregularity Detection & Scopus & Conference \\
    \midrule
    ADG119~\cite{ADG119} & Deep autoencoding models for unsupervised anomaly segmentation in brain MR images & Scopus & Workshop \\
    \midrule
    ADG120~\cite{ADG120} & Anomaly Detection Using GANs for Visual Inspection in Noisy Training Data & Scopus & Conference \\
    \midrule
    ADG121~\cite{ADG121} & An intelligent operation and maintenance system for power consumption based on deep learning & Scopus & Conference \\
    \midrule
    ADG122~\cite{ADG122} & DOPING: Generative Data Augmentation for Unsupervised Anomaly Detection with GAN & Scopus & Conference \\
    \midrule
    ADG123~\cite{ADG123} & Detection of exudates in fundus photographs with imbalanced learning using conditional generative adversarial network & Scopus & Journal \\
    % \midrule
    % ADG124~\cite{ADG124} & Breast cancer detection using synthetic mammograms from generative adversarial networks in convolutional neural networks & Scopus & Journal \\
    \midrule
    ADG124~\cite{ADG124} & Medical image synthesis for data augmentation and anonymization using generative adversarial networks & Scopus & Workshop \\
    \midrule
    ADG125~\cite{ADG125} & CCTV Image Sequence Generation and Modeling Method for Video Anomaly Detection Using Generative Adversarial Network & Scopus & Conference \\
    \midrule
    ADG126~\cite{ADG126} & Chest x-ray generation and data augmentation for cardiovascular abnormality classification & Scopus & Conference \\
    \midrule
    ADG127~\cite{ADG127} & Satellite image forgery detection and localization using GAN and One-Class classifier & Scopus & Journal \\
    \midrule
    ADG128~\cite{ADG128} & Unsupervised anomaly detection with generative adversarial networks to guide marker discovery & Scopus & Conference \\
    \midrule
    ADG129~\cite{ADG129} & Blood flow anomaly detection via generative adversarial networks a preliminary study & Scopus & Conference \\
    \bottomrule
    % \caption{Add caption}
    \end{longtable}%
  \label{tab:longtable}%


==> Sections/Primary_Studies.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'

  \centering
  \tiny

    \begin{longtable}{|c|l|c|c|}
    \caption{Summary of publications.}\\
    \toprule
    \textbf{Study ID} & \textbf{Title} & \textbf{Database} & \textbf{Pub. Type} \\
    \midrule
    ADG01~\cite{ADG01} & IGAN-IDS: An imbalanced generative adversarial network towards intrusion detection system in ad-hoc networks & Science Direct & Journal \\
    \midrule
    ADG02~\cite{ADG02} & Oversampling method using outlier detectable generative adversarial network & Science Direct & Journal \\
    \midrule
    ADG03~\cite{ADG03} & Exploiting the generative adversarial framework for one-class multi-dimensional fault detection & Science Direct & Journal \\
    \midrule
    ADG04~\cite{ADG04} & f-AnoGAN: Fast unsupervised anomaly detection with generative adversarial networks & Science Direct & Journal \\
    \midrule
    ADG05~\cite{ADG05} & Android-GAN: Defending against android pattern attacks using multi-modal generative network as anomaly detector & Science Direct & Journal \\
    \midrule
    ADG06~\cite{ADG06} & Unsupervised automatic seizure detection for focal-onset seizures recorded with behind-the-ear EEG using an anomaly-detecting generative adversarial network & Science Direct & Journal \\
    \midrule
    ADG07~\cite{ADG07} & Energy theft detection in an edge data center using threshold-based abnormality detector & Science Direct & Journal \\
    \midrule
    ADG08~\cite{ADG08} & A System for Spatiotemporal Anomaly Localization in Surveillance Videos & ACM   & Conference \\
    \midrule
    ADG09~\cite{ADG09} & PredGAN: A Deep Multi-Scale Video Prediction Framework for Detecting Anomalies in Videos & ACM   & Conference \\
    \midrule
    ADG10~\cite{ADG10} & Deep Learning-Based Model to Fight Against Ad Click Fraud & ACM   & Conference \\
    \midrule
    ADG11~\cite{ADG11} & Spatial Temporal Balanced Generative Adversarial AutoEncoder for Anomaly Detection & ACM   & Conference \\
    \midrule
    ADG12~\cite{ADG12} & Driving Anomaly Detection with Conditional Generative Adversarial Network Using Physiological and CAN-Bus Data & ACM   & Conference \\
    \midrule
    ADG13~\cite{ADG13} & Anomaly Detection in Traffic Surveillance Videos with GAN-Based Future Frame Prediction & ACM   & Conference \\
    \midrule
    ADG14~\cite{ADG14} & One-Class Classification with Deep Adversarial Learning & ACM   & Conference \\
    \midrule
    ADG15~\cite{ADG15} & Bypassing Detection of URL-Based Phishing Attacks Using Generative Adversarial Deep Neural Networks & ACM   & Workshop \\
    \midrule
    ADG16~\cite{ADG16} & Coupled IGMM-GANs with Applications to Anomaly Detection in Human Mobility Data & ACM   & Journal \\
    \midrule
    ADG17~\cite{ADG17} & Data Augmentation Using Generative Adversarial Networks for Electrical Insulator Anomaly Detection & ACM   & Conference \\
    \midrule
    ADG18~\cite{ADG18} & Sparse-Gan: Sparsity-Constrained Generative Adversarial Network for Anomaly Detection in Retinal OCT Image & IEEE  & Symposium \\
    \midrule
    ADG19~\cite{ADG19} & Anomaly Generation Using Generative Adversarial Networks in Host-Based Intrusion Detection & IEEE  & Conference \\
    \midrule
    ADG20~\cite{ADG20} & Anomaly Monitoring Framework in Lane Detection With a Generative Adversarial Network & IEEE  & Journal \\
    \midrule
    ADG21~\cite{ADG21} & Semisupervised Spectral Learning With Generative Adversarial Network for Hyperspectral Anomaly Detection & IEEE  & Journal \\
    \midrule
    ADG22~\cite{ADG22} & Generative Adversarial Network Based Anomaly Detection on the Benchmark Tennessee Eastman Process & IEEE  & Conference \\
    \midrule
    ADG23~\cite{ADG23} & Memory-Augmented Anomaly Generative Adversarial Network for Retinal OCT Images Screening & IEEE  & Symposium \\
    \midrule
    ADG24~\cite{ADG24} & Anomaly Detection in Time Series using Generative Adversarial Networks & IEEE  & Conference \\
    \midrule
    ADG25~\cite{ADG25} & Finding Anomalies with Generative Adversarial Networks for a Patrolbot & IEEE  & Conference \\
    \midrule
    ADG26~\cite{ADG26} & Anomaly Detection of Railway Catenary Based on Deep Convolutional Generative Adversarial Networks & IEEE  & Conference \\
    \midrule
    ADG27~\cite{ADG27} & Generative Adversarial Networks For Launching and Thwarting Adversarial Attacks on Network Intrusion Detection Systems & IEEE  & Conference \\
    \midrule
    ADG28~\cite{ADG28}& Interpreting Abnormality of a Complex Static Scene using Generative Adversarial Network & IEEE  & Conference \\
    \midrule
    ADG29~\cite{ADG29} & A Generative Adversarial Network Based Framework for Unsupervised Visual Surface Inspection & IEEE  & Conference \\
    \midrule
    ADG30~\cite{ADG30} & Generative Adversarial Networks (GAN) based Anomaly Detection in Industrial Software Systems & IEEE  & Conference \\
    \midrule
    ADG31~\cite{ADG31} & A Generic Anomaly Detection of Catenary Support Components Based on Generative Adversarial Networks & IEEE  & Journal \\
    \midrule
    ADG32~\cite{ADG32} & Discriminative Reconstruction Constrained Generative Adversarial Network for Hyperspectral Anomaly Detection & IEEE  & Journal \\
    \midrule
    ADG33~\cite{ADG33} & What goes around comes around: Cycle-Consistency-based Short-Term Motion Prediction for Anomaly Detection using Generative Adversarial Networks & IEEE  & Conference \\
    \midrule
    ADG34~\cite{ADG34} & Anomaly Detection via Minimum Likelihood Generative Adversarial Networks & IEEE  & Conference \\
    \midrule
    ADG35~\cite{ADG35} & Anomaly Event Detection Using Generative Adversarial Network for Surveillance Videos & IEEE  & Conference \\
    \midrule
    ADG36~\cite{ADG36} & Industrial Anomaly Detection and One-class Classification using Generative Adversarial Networks & IEEE  & Conference \\
    \midrule
    ADG37~\cite{ADG37} & Dual Discriminator Generative Adversarial Network for Video Anomaly Detection & IEEE  & Journal \\
    \midrule
    ADG38~\cite{ADG38} & Unsupervised Multi-Discriminator Generative Adversarial Network for Lung Nodule Malignancy Classification & IEEE  & Journal \\
    \midrule
    ADG39~\cite{ADG39} & 3D Convolutional Generative Adversarial Networks for Detecting Temporal Irregularities in Videos & IEEE  & Conference \\
    \midrule
    ADG40~\cite{ADG40} & Visual Detection of Generic Defects in Industrial Components using Generative Adversarial Networks & IEEE  & Conference \\
    \midrule
    ADG41~\cite{ADG41} & Stock Price Manipulation Detection using Generative Adversarial Networks & IEEE  & Symposium \\
    \midrule
    ADG42~\cite{ADG42} & Generative Adversarial Networks for Distributed Intrusion Detection in the Internet of Things & IEEE  & Conference \\
    \midrule
    ADG43~\cite{ADG43} & Coupled IGMM-GANs for improved generative adversarial anomaly detection & IEEE  & Conference \\
    \midrule
    ADG44~\cite{ADG44} & Survey on Applying GAN for Anomaly Detection & IEEE  & Conference \\
    \midrule
    ADG45~\cite{ADG45} & GAN-Based Anomaly Detection and Localization of Multivariate Time Series Data for Power Plant & IEEE  & Conference \\
    \midrule
    ADG46~\cite{ADG46} & A GAN-Based Anomaly Detection Method for Isoelectric Line in High-Speed Railway & IEEE  & Conference \\
    \midrule
    ADG47~\cite{ADG47} & Mahalanobis Distance Based Adversarial Network for Anomaly Detection & IEEE  & Conference \\
    \midrule
    ADG48~\cite{ADG48} & Fence GAN: Towards Better Anomaly Detection & IEEE  & Conference \\
    \midrule
    ADG49~\cite{ADG49} & A Novel LSTM-GAN Algorithm for Time Series Anomaly Detection & IEEE  & Conference \\
    \midrule
    ADG50~\cite{ADG50} & A GAN-Based Anomaly Detection Approach for Imbalanced Industrial Time Series & IEEE  & Journal \\
    \midrule
    ADG51~\cite{ADG51} & Enhanced Adversarial Learning Based Video Anomaly Detection with Object Confidence and Position & IEEE  & Conference \\
    \midrule
    ADG52~\cite{ADG52} & ADGAN: A Scalable GAN-based Architecture for Image Anomaly Detection & IEEE  & Conference \\
    \midrule
    ADG53~\cite{ADG53} & Generative Adversarial Active Learning for Unsupervised Outlier Detection & IEEE  & Journal \\
    \midrule
    ADG54~\cite{ADG54} & Learning-Based Real-Time Process-Aware Anomaly Monitoring for Assured Autonomy & IEEE  & Journal \\
    \midrule
    ADG55~\cite{ADG55} & Lifelong Disk Failure Prediction via GAN-Based Anomaly Detection & IEEE  & Conference \\
    \midrule
    ADG56~\cite{ADG56} & A Semi-supervised Approach for Steam Turbine Health Prognostics Based on GAN and PF & IEEE  & Conference \\
    \midrule
    ADG57~\cite{ADG57} & Abnormal Chest X-Ray Identification With Generative Adversarial One-Class Classifier & IEEE  & Symposium \\
    \midrule
    ADG58~\cite{ADG58} & Time Series Anomaly Detection Based on GAN & IEEE  & Conference \\
    \midrule
    ADG59~\cite{ADG59} & Anomaly Dataset Augmentation Using the Sequence Generative Models & IEEE  & Conference \\
    \midrule
    ADG60~\cite{ADG60} & Adversarially Learned Abnormal Trajectory Classifier & IEEE  & Conference \\
    \midrule
    ADG61~\cite{ADG61} & Adversarially Learned Anomaly Detection & IEEE  & Conference \\
    \midrule
    ADG62~\cite{ADG62} & A Novel and Efficient CVAE-GAN-Based Approach With Informative Manifold for Semi-Supervised Anomaly Detection & IEEE  & Journal \\
    \midrule
    ADG63~\cite{ADG63} & Training Adversarial Discriminators for Cross-Channel Abnormal Event Detection in Crowds & IEEE  & Conference \\
    \midrule
    ADG64~\cite{ADG64} & Unsupervised Anomaly Detection and Localization Based on Deep Spatiotemporal Translation Network & IEEE  & Journal \\
    \midrule
    ADG65~\cite{ADG65} & MVTec AD — A Comprehensive Real-World Dataset for Unsupervised Anomaly Detection & IEEE  & Conference \\
    \midrule
    ADG66~\cite{ADG66} & Deep Embedding GAN-based Model for Anomaly Detection on High-dimensional Sparse Data & IEEE  & Conference \\
    \midrule
    ADG67~\cite{ADG67} & Robust and Computationally-Efficient Anomaly Detection Using Powers-Of-Two Networks & IEEE  & Conference \\
    \midrule
    ADG68~\cite{ADG68} & GAN Augmented Text Anomaly Detection with Sequences of Deep Statistics & IEEE  & Conference \\
    \midrule
    ADG69~\cite{ADG69} & Abnormal Colon Polyp Image Synthesis Using Conditional Adversarial Networks for Improved Detection Performance & IEEE  & Journal \\
    \midrule
    ADG70~\cite{ADG70} & Defect Image Sample Generation With GAN for Improving Defect Recognition & IEEE  & Journal \\
    \midrule
    ADG71~\cite{ADG71} & Steel Surface Defect Detection Using GAN and One-Class Classifier & IEEE  & Conference \\
    \midrule
    ADG72~\cite{ADG72} & Generative And Encoded Anomaly Detectors & IEEE  & Workshop \\
    \midrule
    ADG73~\cite{ADG73} & Discriminative Autoencoding Framework for Simple and Efficient Anomaly Detection & IEEE  & Journal \\
    \midrule
    ADG74~\cite{ADG74} & Deep Learning Based Fusion of RGB and Infrared Images for the Detection of Abnormal Condition of Fused Magnesium Furnace & IEEE  & Conference \\
    \midrule
    ADG75~\cite{ADG75} & a Multi-Perspective Approach to Anomaly Detection for Self-Aware Embodied Agents & IEEE  & Conference \\
    \midrule
    ADG76~\cite{ADG76} & High Performance WGAN-GP based Multiple-category Network Anomaly Classification System & IEEE  & Conference \\
    \midrule
    ADG77~\cite{ADG77} & Self-Secured Control with Anomaly Detection and Recovery in Automotive Cyber-Physical Systems & IEEE  & Conference \\
    \midrule
    ADG78~\cite{ADG78} & Abnormal event detection in videos using generative adversarial nets & IEEE  & Conference \\
    \midrule
    ADG79~\cite{ADG79} & Learning Normal Patterns via Adversarial Attention-based Autoencoder for Abnormal Event Detection in Videos & IEEE  & Journal \\
    \midrule
    ADG80~\cite{ADG80} & AI-Based Abnormality Detection at the PHY-Layer of Cognitive Radio by Learning Generative Models & IEEE  & Journal \\
    \midrule
    ADG81~\cite{ADG81} & Image-based Process Monitoring via Adversarial Autoencoder with Applications to Rolling Defect Detection & IEEE  & Journal \\
    \midrule
    ADG82~\cite{ADG82} & Bone Metastatic Tumor Detection based on AnoGAN Using CT Images & IEEE  & Conference \\
    \midrule
    ADG83~\cite{ADG83} & Credit Card Transactions Data Adversarial Augmentation in the Frequency Domain & IEEE  & Conference \\
    \midrule
    ADG84~\cite{ADG84} & Data Expansion for Foreign Object Detection in Power Grid & IEEE  & Conference \\
    \midrule
    ADG85~\cite{ADG85} & Adversarially Learned One-Class Classifier for Novelty Detection & IEEE  & Conference \\
    \midrule
    ADG86~\cite{ADG86} & An Adversarial Learning Approach to Medical Image Synthesis for Lesion Detection & IEEE  & Journal \\
    \midrule
    ADG87~\cite{ADG87} & Photoshopping Colonoscopy Video Frames & IEEE  & Symposium \\
    \midrule
    ADG88~\cite{ADG88} & End-to-End Adversarial Learning for Intrusion Detection in Computer Networks & IEEE  & Conference \\
    \midrule
    ADG89~\cite{ADG89} & Assessment of Data Augmentation Strategies Toward Performance Improvement of Abnormality Classification in Chest Radiographs & IEEE  & Conference \\
    \midrule
    ADG90~\cite{ADG90} & Deep detector classifier (DeepDC) for moving objects segmentation and classification in video surveillance & IEEE  & Journal \\
    \midrule
    ADG91~\cite{ADG91} & Multi-sensor Fusion for Magnetic Flux Leakage Defect Characterization Under Information Incompletion & IEEE  & Journal \\
    \midrule
    ADG92~\cite{ADG92} & A Simple Recurrent Unit Model Based Intrusion Detection System With DCGAN & IEEE  & Journal \\
    \midrule
    ADG93~\cite{ADG93} & Relativistic Discriminator: A One-Class Classifier for Generalized Iris Presentation Attack Detection & IEEE  & Conference \\
    \midrule
    ADG94~\cite{ADG94} & Unsupervised Protocol-based Intrusion Detection for Real-world Networks & IEEE  & Conference \\
    \midrule
    ADG95~\cite{ADG95} & An automobile environment detection system based on deep neural network and its implementation using iot-enabled in-vehicle air quality sensors & Scopus & Journal \\
    \midrule
    ADG96~\cite{ADG96} & Unsupervised Anomaly Detection of Healthcare Providers Using Generative Adversarial Networks & Scopus & Conference \\
    \midrule
    ADG97~\cite{ADG97} & video anomaly detection in post-procedural use of laparoscopic videos & Scopus & Workshop \\
    \midrule
    ADG98~\cite{ADG98} & GAN-based Abnormal Detection by Recognizing Ungeneratable Patterns & Scopus & Conference \\
    \midrule
    ADG99~\cite{ADG99} & Semi-supervised Deep Learning for Network Anomaly Detection & Scopus & Conference \\
    \midrule
    ADG100~\cite{ADG100} & MimicGAN: Robust Projection onto Image Manifolds with Corruption Mimicking & Scopus & Journal \\
    \midrule
    ADG101~\cite{ADG101} & Perceptual Image Anomaly Detection & Scopus & Conference \\
    \midrule
    ADG102~\cite{ADG102} & Abnormal Event Detection and Localization in Visual Surveillance & Scopus & Conference \\
    \midrule
    ADG103~\cite{ADG103} & A new GAN-based anomaly detection (GBAD) approach for multi-threat object classification on large-scale x-ray security images & Scopus & Journal \\
    \midrule
    ADG104~\cite{ADG104} & Early Detection of Tomato Spotted Wilt Virus by Hyperspectral Imaging and Outlier Removal Auxiliary Classifier Generative Adversarial Nets (OR-AC-GAN) & Scopus & Journal \\
    \midrule
    ADG105~\cite{ADG105} & Unsupervised anomaly detection system for railway turnout based on GAN & Scopus & Conference \\
    \midrule
    ADG106~\cite{ADG106} & AE-CGAN model based high performance network intrusion detection system & Scopus & Journal \\
    \midrule
    ADG107~\cite{ADG107} & Breast cancer detection using synthetic mammograms from generative adversarial networks in convolutional neural networks & Scopus & Journal \\
    \midrule
    ADG108~\cite{ADG108} & MAD-GAN: Multivariate Anomaly Detection for Time Series Data with Generative Adversarial Networks & Scopus & Conference \\
    \midrule
    ADG109~\cite{ADG109} & LogGAN: A Sequence-Based Generative Adversarial Network for Anomaly Detection Based on System Logs & Scopus & Conference \\
    \midrule
    ADG110~\cite{ADG110} & Image anomaly detection with generative adversarial networks & Scopus & Conference \\
    \midrule
    ADG111~\cite{ADG111} & Few-shot learning with generative adversarial networks based on WOA13 data & Scopus & Journal \\
    \midrule
    ADG112~\cite{ADG112} & Using generative adversarial networks and transfer learning for breast cancer detection by convolutional neural networks & Scopus & Conference \\
    \midrule
    ADG113~\cite{ADG113} & GANomaly: Semi-supervised Anomaly Detection via Adversarial Training & Scopus & Conference \\
    \midrule
    ADG114~\cite{ADG114} & Deep adversarial one-class learning for normal and abnormal chest radiograph classification & Scopus & Conference \\
    \midrule
    ADG115~\cite{ADG115} & Semi-supervised VAE-GAN for Out-of-Sample Detection Applied to MRI Quality Control & Scopus & Conference \\
    \midrule
    ADG116~\cite{ADG116} & Deep learning for automated defect detection in high-reliability electronic parts & Scopus & Conference \\
    \midrule
    ADG117~\cite{ADG117} & Detecting Anomalies in Communication Packet Streams Based on Generative Adversarial Networks & Scopus & Conference \\
    \midrule
    ADG118~\cite{ADG118} & AVID: Adversarial Visual Irregularity Detection & Scopus & Conference \\
    \midrule
    ADG119~\cite{ADG119} & Deep autoencoding models for unsupervised anomaly segmentation in brain MR images & Scopus & Workshop \\
    \midrule
    ADG120~\cite{ADG120} & Anomaly Detection Using GANs for Visual Inspection in Noisy Training Data & Scopus & Conference \\
    \midrule
    ADG121~\cite{ADG121} & An intelligent operation and maintenance system for power consumption based on deep learning & Scopus & Conference \\
    \midrule
    ADG122~\cite{ADG122} & DOPING: Generative Data Augmentation for Unsupervised Anomaly Detection with GAN & Scopus & Conference \\
    \midrule
    ADG123~\cite{ADG123} & Detection of exudates in fundus photographs with imbalanced learning using conditional generative adversarial network & Scopus & Journal \\
    % \midrule
    % ADG124~\cite{ADG124} & Breast cancer detection using synthetic mammograms from generative adversarial networks in convolutional neural networks & Scopus & Journal \\
    \midrule
    ADG124~\cite{ADG124} & Medical image synthesis for data augmentation and anonymization using generative adversarial networks & Scopus & Workshop \\
    \midrule
    ADG125~\cite{ADG125} & CCTV Image Sequence Generation and Modeling Method for Video Anomaly Detection Using Generative Adversarial Network & Scopus & Conference \\
    \midrule
    ADG126~\cite{ADG126} & Chest x-ray generation and data augmentation for cardiovascular abnormality classification & Scopus & Conference \\
    \midrule
    ADG127~\cite{ADG127} & Satellite image forgery detection and localization using GAN and One-Class classifier & Scopus & Journal \\
    \midrule
    ADG128~\cite{ADG128} & Unsupervised anomaly detection with generative adversarial networks to guide marker discovery & Scopus & Conference \\
    \midrule
    ADG129~\cite{ADG129} & Blood flow anomaly detection via generative adversarial networks a preliminary study & Scopus & Conference \\
    \bottomrule
    % \caption{Add caption}
    \end{longtable}%
  \label{tab:longtable}%

